Technical Report: Insider-Resistant Context-Based Pairing for Multimodality Sleep Apnea Test

The increasingly sophisticated at-home screening systems for obstructive sleep apnea (OSA), integrated with both contactless and contact-based sensing modalities, bring convenience and reliability to remote chronic disease management. However, the device pairing processes between system components are vulnerable to wireless exploitation from a non-compliant user wishing to manipulate the test results. This work presents SIENNA, an insider-resistant context-based pairing protocol. SIENNA leverages JADE-ICA to uniquely identify a user's respiration pattern within a multi-person environment and fuzzy commitment for automatic device pairing, while using friendly jamming technique to prevents an insider with knowledge of respiration patterns from acquiring the pairing key. Our analysis and test results show that SIENNA can achieve reliable (> 90% success rate) device pairing under a noisy environment and is robust against the attacker with full knowledge of the context information.

==> src/sections/acknowledgement.tex <==
This work is supported in part by the National Science Foundation (NSF) under grants IIP-1831303, IIS-1915738, and CNS-1948568, as well as the equipment from TMYTEK mmWave research initiative.

==> src/sections/analysis_conf.tex <==
The security of SIENNA can be formally analyzed based on the property of a fuzzy commitment, and extended into three cases according to the attacker's knowledge on the user's breathing fingerprint, $f$. In the following, we omit the proof of the first two cases and focus on the third one to conserve space\footnoteref{tech_report}.

{\bf Attacker without Knowledge of $f$.} When the eavesdropper does not have the correct context, SIENNA inherits the security properties of a fuzzy commitment, in terms of concealment and binding \cite{JuelsFuzzyCommitmentScheme1999}.


{\bf Attacker with General Knowledge of $f$.} 
By knowing the distribution of $f$, the attacker can have computationally less expensive strategies to determine $\hat{l}$. One way to enhance SIENNA's security is to commit and decommit $l$ via multiple samples/segments of $f$ as shown in Section \ref{section:respiration fingerprinting}. Yao's XOR lemma \cite{GoldreichYaoXORlemma2011} indicates that the attacker's advantage due to bias in $f$'s distribution diminishes as we increase the number of $f$s in the XOR chain, with the diminishing rate defined in \cite{GoldreichYaoXORlemma2011}.


% \begin{figure*}[ht]
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/AlvinAlone.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/AlvinThomasClose.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/AlvinThomasFar.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Substitute.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Eavesdropper.png}
% \end{subfigure}
% \caption{Left to right: (a) One person scenario for compliance tracking with patient; (b) Mix-up: patient lies together with non-patient in close distance; (c) Mix-up: patient lies separately with non-patient; (d) Surrogate: radar tracks non-patient; (e) Eavesdropper records signal from radar.}
% \label{fig:experiment set-up}
% \end{figure*}

{\bf Attacker with Perfect Knowledge of $f$.}
The XOR-chain trick would not prevent an attacker with perfect knowledge of $f$ to retrieve $s$. For a malicious patient capable of measuring his own breathing patterns. When he is also able to capture the commitment message, $\{c, \mathcal{H}(s)\}$, he can accurately compute $l = c  \ominus f$ and decode to obtain $s$. 

% \begin{figure*}[t]
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig-4-journal-2.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth]{figures/FONTS_PLEASE.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig9_BW.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/slant-ranges-fingerprint-similarity-most-recentt.eps}
% \end{subfigure}
% \caption{Left to right: (a) Multiple vital related dynamic features, including breathing rate, inhale/exhale area, breathing depth, and heart rate, are preserved after level-crossing quantization; (b) The distributions of fingerprint similarity between chestband-based and mmWave-based modalities, captured from the same subject; (b) The distributions of fingerprint similarity between chestband-based and mmWave-based modalities, captured from different subjects (chestband data from the patient, mmWave radar data from the non-patient); (d) The effect on the fingerprint similarity due to the change of slant range between the mmWave radar and the subject.}
% \label{fig:fingerprint extraction}
% \end{figure*}

\begin{figure*}[t]
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth,height=\textwidth]{figures/feature_preservation.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/friend_similarity.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth,height=\textwidth]{figures/attack_similarity.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth,height=\textwidth]{figures/friendly_jamming.eps}
\end{subfigure}
\caption{Left to right: (a) Signal reconstructed after 64-level-crossing quantization with vital related dynamic features preserved; (b)  Similarity between belt-based and PRMS-based breathing patterns, measured with the same subject; (c) Similarity between belt-based and PRMS-based breathing patterns, measured with different subjects; (d) Performance of SIENNA against eavesdropper with full knowledge of breathing patterns, measured in aggregated BER.}
\label{fig:key evolution}
\vspace{-15pt}
\end{figure*}

To prevent such an insider attack, SIENNA leverages friendly jamming to obfuscate the commit message for any unintended receivers, and we can analyze the security of it based on a wiretap channel model \cite{LiangCompoundWiretapChannels2009}. Consider a non-compliant patient using an unauthorized receiver to intercept the commit message $X$. We denote the main channel as the wireless channel between $a$ and $b$ and the wiretap channel as the one between the unauthorized receiver and $a$ or $b$. 
Then the frequency-domain representation of the main channel and the wiretap channel is,
\begin{align*}
    & Y_{\text{main}} = X + \frac{P_0}{P_1}\mathcal{N}(0, \sigma^2_0), & Y_{\text{tap}} = X + \frac{P}{P_2}\mathcal{N}(0, \sigma^2)
\end{align*}
respectively, where $P_0$ and $\sigma^2_0$ denote the average power and variance of the intrinsic wireless noise, $P_1$ and $P_2$ denote the average powers of the OFDM signal observed by the receiver and the unauthorized receiver, and $P$ and $\sigma^2$ denote average power and variance of the jamming signal observed by the unauthorized receiver. 

\cite{GollakotaPhysicalLayerWireless2011} has shown that the jamming scheme works at its optimal when the OFDM system operates with high order modulation (at least QPSK), and $1 < P/P_2 < 9$.\footnote{The jamming signal is too weak to degrade the OFDM signal when $P/P_2 \leq 1$, and too strong to be indistinguishable from the OFDM signal when  $P/P_2 \ge 9$.} Therefore, SIENNA prohibits the transmit in BPSK at any SNR. Due to the FFT/IFFT operations in the OFDM system, $X$ is a pseudorandom Gaussian signal according to the central limit theorem. The bit error probability for such an OFDM system, allowing only M-QAM transmission, is 
\[
B_{\text{main}} \simeq \frac{4}{\log_2{M}}\textsc{Q}\left( \sqrt{\frac{3 P_1 \log_2{M}}{P_0(M-1)}} \right)
\]
for the main channel and 
\[
B_{\text{tap}} \simeq \frac{4}{\log_2{M}}\textsc{Q}\left( \sqrt{\frac{3 P_2 \log_2{M}}{P(M-1)}} \right),
\]
for the wiretap channel, where $\textsc{Q}(\cdot)$ denotes the the tail distribution function of the standard normal distribution. The receiver may adjust $P$ to elevate $B_{\text{tap}}$ beyond the error correction capability of the fuzzy commitment, and prevent an insider attack. The issue is that the jamming is only effective when $1 < P/P_2 < 9$, but $P_2$ depends on the location of the unauthorized receiver and is unknown to the receiver. Our solution is to have the transmitter create $L$ commitments, each with one sub-salt, and transmit them one by one, while the receiver jams at $L$ different power levels, $\{P_{\text{max}}, P_{\text{max}}/9, \ldots, P_{\text{max}}/9^{L-1}\}$. Given the fact that $B_{\text{main}}$ is not affected by $P$, the receiver can recover all sub-salts and XOR them together to obtain the key evolution salt. In contrast, the unauthorized receiver will fail to decode at least one sub-salt, therefore, cannot recover the key evolution salt. The number of jamming levels, $L$, can be computed based on the upper bound (the maximum power supported by the hardware, $P_{\text{max}}$) and lower bound (the noise floor, $P_0$) on the OFDM signal power. 

==> src/sections/evaluation_conf.tex <==
We empirically evaluated the performance of SIENNA, which consists of a PRMS implemented with mmWave transceivers/radio heads, one respiratory belt sensor implemented with a piezo-electric respiration transducer, and one Android-based OSA application. We conducted laboratory and field experiments over one month with the SIENNA prototype and 20 subjects selected through a random sample recruitment process. All experiments with human subjects are approved by the Institutional Review Board (IRB) based on the written consent.

We designed the eavesdropping and spoofing attacks with BLE sniffer and spoofer, implemented via Ubertooth and Kismet. During each experiment, the subject was asked to wear a respiratory belt and lie under a PRMS. A third party manually executes the pairing process, and the packets communicated between the mobile OSA app and the PRMS were identified based on their Bluetooth Device Addresses (BDAs) obtained before the experiment. During the eavesdropping attack, the host's codes on the BLE sniffer record the packets containing the fuzzy commitment, which were analyzed offline to deduce the keys. During the spoofing attacks, an attacker-generated compliance tracking data encrypted with the deduced key was transmitted at higher power when the PRMS uploads the data to the mobile OSA app to manipulate the latter into accepting the fraudulent data, which was verified during offline analysis.

SIENNA's performance against eavesdropping and spoofing is evaluated by comparing the aggregated bit error rate (BER) at the receiver versus the aggregated BER at the attacker side. Due to the application of fuzzy commitment, the key establishment protocol allows a maximum of 27\% BER in the breathing fingerprints (when using $(2^8, 255, 201)$ Reed-Solomon codes) to recover the key salt. Compared to Fig. \ref{fig:key evolution}c, such a BER alone prevents any outside attackers who cannot observe and mimick the patient's breathing patterns from stealing the key salt. Our experiment further showed that the jamming signal could suppress the attacker's BER to approximately 50\% within the PRMS's transmission range (Fig. \ref{fig:key evolution}d). The CDF of the accumulated BERs for attackers at any locations within the PRMS's transmission range concentrated between 41\% to 50\% (Fig. \ref{fig:key evolution}d) and is well beyond the correctable range of the selected Reed-Solomon codes.

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.75\linewidth]{figures/smartphone.png}
% \caption{Implementation of MASCOT with, an Android application, a chestband sensor, and mmWave Radar.}
% \label{fig:system implementation}
% \end{figure}

% \begin{figure*}[t]
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Figure_8_A_Test_New.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Figure_8_B_Test_new.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig-7-journal-2.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig-3-journal-2.eps}
% \end{subfigure}
% \caption{Left to right: (a) Raw IQ data received by different RF channels of the the mmWave CW radar in Fig. \ref{fig:experiment set-up}b; (b) Breathing mixture obtained by (linear) demodulating the raw IQ (top), individual breathing patterns after source separation in comparison with the ones collected by the chestband sensor (bottom); (c,d) time and frequency domain analysis show the inhale and exhale characters are distinct between the two subjects, which allows patient tracking during modality switches.}
% \label{fig:breathing separation}
% \end{figure*}

% \subsection{Implementing MASCOT}
% Our MASCOT prototype was developed and tested from 2019 to 2020, with two mmWave radars implemented for the preliminary system. The first design employs a commercial off-the-shelf 4-channel 24GHz monopulse radar transceiver (K-MC4 from RFbeam Microwave GmbH) interfacing a LabVIEW controlled DAQ through four LNA's (SR560 from Stanford Research System). The 3dB beam aperture is $12^{\circ}$ horizontally and $30^{\circ}$ vertically. The angle coverage is between +/-$15^{\circ}$ horizontally. The second design, aiming to address the reflection noise issue identified with the first design, is a customized 14/28GHz harmonic monopulse radar implemented via a mmWave beamforming development kit (BBox one/UD box from TMYTEK). The kit consists of a 16-channel 24-31GHz phased array antenna, and a frequency Up/Down converter, which interfaces with a LabVIEW controlled USRP (USRP-2974 from NI). The 3dB beam aperture is $13^{\circ}$ horizontally and $14^{\circ}$ vertically. The angle coverage is +/-$45^{\circ}$ horizontally and +/-$60^{\circ}$ vertically. The harmonic function is implemented via an analog frequency divider at the TX, and a miniature harmonic transponder (diode based frequency doubler, fabricated at OSH Park) attached to the patient.

% The skin-contacting compliance tracker is implemented with a piezo-electric respiration transducer (Model 1132 Pneumotrace II from UFI), which interfaces with a LabVIEW controlled DAQ. The Android application communicates via Bluetooth Low Energy (BLE) with the host computers that control the mmWave radar(s) and the respiration transducer to execute the modality-switching and data logging functionality. The implementation leverages the Android BLE APIs to connect to the Generic Attribute Profile (GATT) servers set up by the LabVIEW Bluetooth Toolkit on the host computers. The physical layer jammer for the chestband sensor is implemented via the Android application connecting to a Wi-Fi-BT-Bluetooth LE breakout board (ESP32-WROVER-IB from ESPRESSIF). The jammer for the mmWave radar is implemented via with a LabVIEW controlled USRP (USRP-2974 from NI).

% \begin{figure*}[t]
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig-4-journal-2.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth]{figures/FONTS_PLEASE.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/Fig9_BW.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.24\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/slant-ranges-fingerprint-similarity-most-recentt.eps}
% \end{subfigure}
% \caption{Left to right: (a) Multiple vital related dynamic features, including breathing rate, inhale/exhale area, breathing depth, and heart rate, are preserved after level-crossing quantization; (b) The distributions of fingerprint similarity between chestband-based and mmWave-based modalities, captured from the same subject; (b) The distributions of fingerprint similarity between chestband-based and mmWave-based modalities, captured from different subjects (chestband data from the patient, mmWave radar data from the non-patient); (d) The effect on the fingerprint similarity due to the change of slant range between the mmWave radar and the subject.}
% \label{fig:fingerprint extraction}
% \end{figure*}

%\subsection{Experiment Setup}
% We conducted laboratory and field experiments over a one-month period with the MASCOT prototype and 20 subjects selected through a random sample recruitment process. The subjects are between the ages of 16 and 35, weigh between 42 to 85 kilograms, and have no prior history of heart disease. The subjects are asked to participate in multiple trials of sleep studies under laboratory and everyday settings with environmental and adversarial complications detailed below.

% \textbf{Sleep Environment and Data Collection.} We furnished two sleep environments for experimentation. The indoor laboratory environment consists of 2 twin size beds under a quiet and dim ambience. The outdoor field environment consists of two beach mats and umbrellas set up at a local beach park. During each trial, the subjects are attached with chestband sensors and positioned 0.5 meters below the mmWave radar system for data collection. We continuously monitor the respiration of the subjects for 1 hour, during which modality-switches and adversarial activities (if planned) are attempted every 10 minutes. After the experiment, we extract a 60-second data segment around each modality-switch to evaluate MASCOT's performance, with the remaining data to serve as references. Overall, we collected approximately 30,000 breathing cycle samples for each subject.

% \textbf{Mix-Up/Surrogate.} We designed the mix-up and surrogate scenarios via a single-blind experiment set-up. For the mix-up scenario, we randomly paired subjects, asked both of them to wear chestbands and lay down under a mmWave radar, without telling which one should act as the patient. A third-party executed the modality switches via the OSA application paired with the patient's chestband and the mmWave radar. For the surrogate scenario, we selected pairs of subjects with similar physiques, asked both of them to wear chestbands but lay down under two separate mmWave radars, without telling which subject was the patient. The surrogate attack was implemented in the following ways: (1) During modality switch, a third-party executed the switches via the OSA application paired with the patient's chestband and the non-patient's mmWave radar. (2) During chestband modality, a third-party disconnected the patient's chestband from the DAQ and connected the non-patient's chestband to the DAQ. (3) During radar modality, a third-party team swapped the two mmWave radars.

% \textbf{Eavesdrop/Spoof.} We designed the eavesdropping and spoofing attacks via a BLE sniffer and spoofer, implemented via Ubertooth and Kismet. During each experiment, one subject was asked to wear a chestband and lay down under a PRMS. A third-party manually execute the pairing process. The packets communicated between the mobile OSA app and the PRMS  were identified based on their Bluetooth Device Addresses (BDAs) obtained prior of the experiment. To implement the eavesdropping attack, the host's codes recorded the packets containing the fuzzy commitment and hash value of the new key during each modality-switch, which were analyzed offline in attempt to deduce the keys. To implement the spoofing attacks, an attacker-generated compliance tracking data encrypted with the deduced key was transmitted at higher power during data upload toward the OSA app, in attempt to manipulate the latter into accepting the fraudulent data, which was verified during offline analysis.


% \subsection{Performance of Breathing Separation}
% During each experiment, the signal (mixture) captured by the PRMS (Fig. \ref{fig:breathing separation}a) was filtered in real-time by the ICA-JADE-based breathing separation module implemented through a MATLAB script running within LabVIEW. The script filtered the signal with a digital FIR Low pass filter with cut off frequency of 10 Hz to suppress the high-frequency noise while preserving the physiological-related information. The filtered signal was linearly demodulated to compute the phase shifts caused by the displacement(s) of the chest(s) surface(s) during breathing (Fig. \ref{fig:breathing separation}b top). Specifically, the script calculated the covariance matrices of the I and Q channel signals and applied eigenvalue decomposition to the covariance matrices to extract the maximum chest displacement information. The demodulated signal was separated by the ICA-JADE method to isolate individual respiratory signatures (Fig. \ref{fig:breathing separation}b bottom). 

% Finally, the script evaluated the performance of ICA-JADE by computing the cross-correlation between the isolated signatures with the ground truth obtained from the respiration transducer. The empirical result shows that the similarity is above 90\% when we limit the experiment within 60 seconds. As time increases, the subjects tend to move/turn on the bed, which changes the contribution of their breathing to the signal mixture, e.g., the mixing matrix, and the ICA-JADE result deviates from the truth. Thus, we limited the sensing period of MASCOT during the subsequent experiments to within 60 seconds to achieve a stable source separation.


% \subsection{Performance of Fingerprint Extraction}
% An individual breathing signature was quantized in parallel by multiple level-crossing LabVIEW VIs to generate the binary fingerprint after breathing separation. The breathing signature (torso deformation) due to respiratory movements is a complex three-dimensional pattern, and varies greatly with subject parameters and activity context. Based on our preliminary data, the thorax motions due to respiration and heartbeat are limited within +/-0.5cm and +/-0.05cm (Fig. \ref{fig:fingerprint extraction}, and the rates of respiration and heartbeat are below 15 and 60 per minute, when the subject is at rest. Therefore, we employed ten level-crossing quantization branches with a quantization step size of 0.05cm at a sample rate of 10 per second, to preserve the fine-grained respiratory motion when extracting the breathing fingerprint.

% To be compatible with the key evolution protocol, the quality of the binary fingerprints was evaluated based on the Hamming distances between fingerprints of the same subject observed by different modalities and different subjects observed by different modalities. It has been demonstrated in various works that human subjects can be sufficiently differentiated based on the inhales (local maxima), exhales (local minima), and breathing depth (the area between two consecutive maxima and in between one minima point). The similarities of these features directly translate to the Hamming distances between the quantized fingerprints. Therefore, comparing the Hamming distances is equivalent to constructing an equal-weighted linear classifier for patient identification.

% The empirical results (Fig. \ref{fig:fingerprint extraction}b) show that the average Hamming similarity per bit between fingerprints of the same subject observed from different modalities is around 63\% when extracted from 6-second breathing signatures (with 2 breathing cycles). The Hamming similarity increases almost logarithmically towards 100\% as we extend the duration of the breathing signature to 60 seconds (with 20 breathing cycles). The elevated mean and reduced variance in the Hamming similarity is mostly due to the extended time, which allows repeated measurements of the periodic respiratory effort motion unique to each subject. 

% On the contrary, the average Hamming similarity per bit between different subjects' fingerprints remains below 5\% despite the measurement duration (Fig. \ref{fig:fingerprint extraction}b). The position between the mmWave and the subject also poses a significant factor, which attenuates the Hamming similarity. As the subject moves away from the radar's downrange direction, the radar measurements deviate from the ground truth (obtained from the chestband). But their similarity remains sufficiently high compared to the breathing fingerprints between different subjects. Overall, the results show that the Hamming similarity per bit for MASCOT can be set to around 70\% to allow accurate patient tracking during modality switches.


% \subsection{Performance of Key Evolution}
% The binary breathing fingerprints, are chunked into multiple 10-second segments and padded with 0s to meet the codeword length of the $(2^{8}, 255, n)$ Reed-Solomon codes, e.g., $8 \times 255 = 2040$ bits. The particular group of Reed-Solomon codes are chosen to ensure the communicated data can be measured in exact multiple of bytes (8 bits). A key evolution salt of $8 \times n$ bits is randomly selected by the on-duty sentinel and encoded with the $\textsc{RS}(2^{8}, 255, n)$ Reed-Solomon encoder to generate the 2040 bits opening value. The opening value and the (multiple) padded fignerprint segments are XORed together to generate the 2040 bits commitment.

% We evaluate the security of the fuzzy commitment via a randomness test using the NIST statistical test suite. Based on 10 million randomly generated key evolution salts (with entropy per bit equal to one), we measured the randomness of the opening values and the commitments (Fig. \ref{fig:key evolution}a). The empirical test shows that the entropy per bit drops almost by half when the key salt is converted into a commitment. In other words, the entropy of a 2040-bit commitment is approximately 1000 bits. The primary causes of the reduction are due to the redundancy in the Reed-Solomon codes and the human respiratory motion's cyclic character. Two additional factors that affect the randomness of the commitment are the quantization levels and the number of the XOR operation rounds. When the quantization levels increase, the granularity of the binary sequencing improves, slightly elevating the randomness of the breathing fingerprints, resulting in a higher degree of entropy in the commitments. When the commitment is generated with multiple rounds of XOR operations, the entropy decreases due to the cross-correlation between fingerprint segments\footnote{In an XOR operation, the higher correlation between the inputs, the less the entropy in the output.}.

% We further measured the commitment and reconstruction time of the key evolution protocol. As the binary quantization takes negligible time to perform, the Reed-Solomon encoder and decoder's efficiency, besides communication delay,  dominates the protocol's turnaround time. We timed our LabVIEW-based protocol implementation with different parity symbol lengths, $k = 255 - n$, in the $(2^{8}, 255, n)$ Reed-Solomon codes. The results show that the overall commitment time is below 0.3 seconds and grows linearly to the maximum number of correctable symbols, $k/2$, due to the additional Lagrange interpolations needed to compute the parity symbols (Fig. \ref{fig:key evolution}b). The overall reconstruction time is below 0.02 seconds and grows linearly to $k/2$, due to the additional syndromes computed for error corrections (Fig. \ref{fig:key evolution}c). The decoding time is invariance to the number of errors in the codewords, which is a security advantage as the attacker cannot infer the decoded message's correctness based on decoding time.

% \subsection{Performance under Adversarial Settings}
% MASCOT's performance against mix-up and surrogate scenarios is assessed based on the protocol's sensitivity (true positive rate) and specificity (true negative rate) in identifying intentional or unintentional identity changes. MASCOT leverages a support vector machine (SVM) to detect identity changes (as anomalies in breathing patterns) within a single modality recording and rely on the success/failure of the key evolution to detect identity changes during modality switches. The overall sensitivity and specificity are calculated as the average among single modality and modality switching cases. Our implementation ensures a fair comparison between fuzzy commitment and SVM by using a linear SVM, whose decision boundary can be interpreted as a weighted Hamming distance between binary breathing fingerprints. The empirical results show that the MASCOT' scores are close to the single modality SVM approach, lower by 1.1\% and 1.5\% in sensitivity and specificity. The performance of single modality SVM approach is close but not precisely 100\%, due to the variance of human respiratory motions. Not that single modality contact-based methods can achieve 100\% detection accuracy if more rigid rules, such as prohibiting sensor disconnection, are enforced through the hardware. However, the detrimental effect of contact sensor toward the quality of the OSA screening data renders it inferior to MASCOT, as discussed in Sec. \ref{sec:background}.

% SIENNA's performance against eavesdropping and spoofing is evaluated by comparing the aggregated bit error rate (BER) at the receiving sentinel versus the aggregated BER at the attacker. Due to the application of fuzzy commitment, the key evolution protocol allows a maximum of 27\% BER in the breathing fingerprints (when using $(2^8, 255, 201)$ Reed-Solomon codes) to recover the key salt. Such BER alone prevents any outsider attackers who cannot observe and mimick the patient's breathing fingerprint from stealing the key salt. Our experiments further showed that the jamming signal could suppress the attacker's BER to approximately 50\% anywhere within the on-duty sentinel's transmission range, rendering the modality-switching message undecidable, even if an attacker could obtain the patient's breathing fingerprint. Overall, the CDF of the accumulated BERs for any attackers concentrated between 41\% to 50\%, well beyond the correctable range of the selected Reed-Solomon codes. Thus, the combination of both techniques ensures sufficient and complete protection of the security key during modality-switching against both outsider and insider attacks.

==> src/sections/intro_conf.tex <==
Over twenty-five million adults in the US suffer from obstructive sleep apnea (OSA), an airway muscle-related breathing condition that involuntarily causes respiratory cessations during sleep. Poor treatment can lead to excessive daytime fatigue, high blood pressure, cardio-metabolic conditions, along with a myriad of health problems \cite{baboli_good_2015}. A traditional diagnostic procedure, known as polysomnography (PSG), requires the patient to be in a laboratory overnight with instruments of multiple sensors/electrodes to track various sleep-related physiological parameters. However, PSG is highly obtrusive, expensive, and scarce.

At-home OSA monitoring systems leverage contactless and/or contact-based sensing technologies to monitor respiratory symptoms related to OSA. They allow users to conduct self-administered tests prescribed by their doctors and are considered economical alternatives for PSG. However, At-home OSA tests are subject to test fraud, as several professions within the patient population are deeply concerned that positive OSA test results will jeopardize their careers. As a result, an OSA patient may exploit the unsupervised at-home environment to manipulate the OSA test results. Specifically, the device pairing processes between the OSA screening system components are often the target of eavesdropping and spoofing from a non-compliant user.  

% To reduce the any low-demanding and less expensive diagnostic procedures have been proposed, studied, and commercialized to bridge the gap between effectiveness and accessibility of sleep tests.

% The extensive medical cost for OSA is due to the diagnostic procedure, known as polysomnography (PSG), which places a patient within a laboratory overnight and instrument the subject with multiple sensors/electrodes to track various sleep-related physiological parameters.

% The medical gold standard for diagnosing sleep apnea is by polysomnography (PSG), where the patient is attached to variety of sensors to record sleep activity overnight. However, PSG is also highly obtrusive, expensive, impractical for home-based use, and can inflict discomfort for patients. 

% Non-contact physiological radar monitoring systems (PRMSs), based on Continuous Wave (CW) Doppler radar, is a promising alternative for at-home sleep tests. Nevertheless, single-modality methods are bounded by the patient's vital signals during sleep tests, and recording ceases as soon as the compliance tracking sensor is detached from the patient. 

% Recent studies on multi-modality, such as wireless sensing and vital-based verification, has shown that heartbeat and respiration dynamics extracted from wireless radio signals are relatively distinguishable among individuals. Breathing patterns can depend on tidal volume, airflow profile, breathing depth, and energy \cite{benchetrit_breathing_2000}, all of which are retrieved through an OSA screening data \cite{IslamIdentityAuthenticationOSA2020}. However, patient identity verification remains susceptible to attackers who can eavesdrop and intercept using contactless and contact-based single-modality methods. As a result, it is necessary to introduce an additional system component to secure the multi-modality framework.

To combat these malicious behaviors, we introduce SIENNA: in\textbf{SI}der r\textbf{E}sista\textbf{N}t co\textbf{N}text-based p\textbf{A}iring for unobtrusive at-home OSA screening. SIENNA works with a multi-modality OSA screening system consisting of one data aggregate, e.g., the user's mobile phone, and two sensing modalities, e.g.,  a respiratory belt and a physiological radar monitoring system (PRMS). It leverages the respiration patterns collected by the respiratory belt to allow automatic pairing between the PRMS and the phone. The design of SIENNA uses a novel combination of JADE-ICA \cite{rutledge_independent_2013}, fuzzy commitment, \cite{JuelsFuzzyCommitmentScheme1999}, and friendly jamming \cite{AroraDialogCodesSecure2009,GollakotaPhysicalLayerWireless2011, MelcherIJamChannelRandomization2020}. The JADE-ICA allows the PRMS to identify the unique patterns of a person's breathing from a multi-person environment. The fuzzy commitment leverages the user's breathing patterns to establish a shared secret key between the PRMS and the mobile phone. And the friendly jamming prevents insiders, e.g., a non-compliant and unsupervised user with knowledge of the breathing patterns, from learning the security key.

We formally analyzed the security of SIENNA based on the attacker's knowledge of the context information, and implemented a laboratory prototype consisting of a mmWave PRMS (implemented with SDR and mmWave radio heads), a wireless respiratory belt, and a Android-based OSA app. We conducted an evaluation consisting of 20 subjects spanning over one month. The results show that SIENNA achieves reliable device pairing within a noisy at-home environment with multiple free moving persons in the background. It also prevents unauthorized receivers from retrieving the secret key, regardless of their locations or knowledge of the user's respiration patterns.\footnote{\label{tech_report}More details can found in our technical report:  \href{http://arxiv.org/abs/2105.00314}{arXiv:2105.00314v1}}.

%The rest of the paper is organized as follows. First, in Section \ref{sec:background}, an overview of Doppler radar and non-contact OSA screening, as well as a description of work relevant to compliance monitoring and identity verification are presented. An introduction and an analysis of the system and adversary models of multi-modality compliance tracking are provided  Section \ref{sec:challenges}. Next, the design of MASCOT is described in Section \ref{sec:mascot} and its security characteristics are analyzed in Section \ref{sec:security_analysis}. Implementations and experimentation of MASCOT are documented in Section \ref{sec:evaluation}. And we conclude in Section \ref{sec:conclusion} with a dicussion of future work.

%To the best of our knowledge, our work is the first attempt to achieve secure radio-based multi-subject identity verification for at-home OSA screening, by harnessing the combined power of Doppler radar and Fuzzy key Extractor.

==> src/sections/keywords.tex <==
telemedicine,
telehealth,
remote healthcare,
non-contact sleep monitoring,
test compliance,
test fraud,
wireless security,
identity verification,
continuous authentication,
continuous wave radar,
harmonic radar,
backscatter radar,
mmWave radar,
mmWave sensing,
fast Fourier transform,
independent component analysis, 
joint approximate digaonalization of eigenmatrices,
support vector machine,
fuzzy commitment,
key derivation,
error-correcting codes,
digital lockers,
wireless physical layer security,
friendly jamming

==> src/sections/radar_primer.tex <==
Here we provide an overview the fundamental of Continuous Wave (CW) Doppler radar theory, which enables the applications of at-home uuobtrusive sleep apnea screening. Physiological monitoring based on mmWave CW Doppler radar have been used to study sleep related disorders, such as sleep apnea. The symptoms of sleep apnea usually involve stoppages in respiration that wakes patients over night. These temporary stoppages are abnormalities in respiratory rhythm that are visible by observing a patient's chest and abdominal movements. When a sleep apnea event occurs, the patient's normal inhale and exhale patterns are interrupted, and his/her chest and abdomen cease to expand or contract for a short period due to a lack of motions from the diaphragm and intercostal muscles. These stasis can be detected by a mmWave CW Doppler radar installed above the bed with its aperture facing the mattress, as shown in (Figure -Yao).

During the sleep study, the radar detects the tiny movements of the patient's chest surface through the phase shift of the reflected signal \cite{droitcour_microwave_2001,lin_microwave_1992,chen_x-band_1986,lin_noninvasive_1975,greneker_radar_1997,droitcour_non-contact_2009,singh_data-based_2013}. Mathematically, the CW Doppler radar signal can be demodulated into two orthonormal channels, in-phase (\textit{I}) and quadrature phase (\textit{Q}). Let the distance offset due to chest movements be $x(t)$, the two channels can be expressed as \cite{park_arctangent_2007}:
\begin{align*}
  {B}_I(t) &= A_I\cos\left(\theta_0+\frac{4\pi x(t)}{\lambda}+\delta\theta(t)\right)\\
  {B}_Q(t) &= A_Q\sin\left(\theta_0+\frac{4\pi x(t)}{\lambda}+\delta\theta(t)\right),
\end{align*}
Where $\lambda$ is the signal wavelength, $\theta_0$ is the phase delay due to the nominal distance between the radar transmitter and the patient's torso, surface scattering, and radar's RF chains, $\delta\theta(t)$ is the residual phase noise. The phase shift corresponds to the respiratory movement can be computed via arctangent demodulation \cite{park_arctangent_2007}:
\begin{equation*}
  \theta(t) = \theta_0 + \frac{4\pi x(t)}{\lambda} = \arctan \left(\frac{A_I{B}_Q(t)}{A_Q{B}_I(t)}\right).
\end{equation*}
Visually, the respiratory motion, $\theta(t)$, swings around the origin on the I-Q plot with the apnea arcs shorter than the arcs due to normal breathing. Viewed on either the I-t or Q-t plots,  $\theta(t)$ fluctuates for normal breathing and remains relatively constant during apnea intervals.

\begin{figure}[h]
\includegraphics[width=0.8\textwidth]{figures/doppler_radar.eps}
\caption{radar primer}
\label{fig:radar primer}
\end{figure}

% A Doppler radar system can operate in an entirely non-contact fashion or in combination with a passive harmonic tag to monitor a patient's respiration. In the former case, the radar system transmits an RF signal and observes the reflection signal at the same frequency, which is modulated by the motion of the human chest. In the latter case, a planar harmonic tag, consisting of a non-linear diode device, is attached to the patient's chest. When energized, the tag emits reflections at the harmonic frequencies of the transmit signal, which can be observed by the radar's receiver toned to those frequencies (citation -Yao). Since there exist few non-linear devices in a natural environment, the harmonic radar technique is capable of suppressing all other RF interference due to the background features.

==> src/sections/related_works.tex <==
The following section provides a brief survey on test compliance tracking, radio-based sensing/verification and co-presence authentication.

\subsection{Test Compliance Tracking}

The OSA test compliance tracking works as follows: Prior to the test, the doctor secures a tracker to the identified patient. Once attached, the tracker continuously observes and records the patient's vital signs until the test is finished. During the follow-up visit, the compliance data is compared with the screening data recorded by the OSA test equipment. If there were significant gaps, during which the compliance tracker fails to observe the patient's vital signs or significant inconsistency between the compliance data and the OSA screening data, the test would be nullified. The initial assessment ensures the patient never removes the tracker, and the subsequent data analysis verifies the identification information between the patient wearing the tracker and subject undergoing the test. 

Existing industry solutions utilize skin-contacting sensors to execute test compliance tracking \cite{noauthor_httpspatentsgooglecompatentus8679012b1en_nodate, noauthor_httpwwwsleepreviewmagcom201806tech-fraudulent-sleep-data_nodate}. These approaches are reliable and have minimal chance of false identifications. However, the patient may feel discomfort due to the attached sensors, which hampers the confidence of the test results. Several relevant experiments achieve identity verification by remotely monitoring and verifying the subject's physiological or behavioral traits. Common methods use imaging or audio sensors to perform facial-based or voice-based recognition \cite{hutchison_robust_2005, li_sound-based_2010,abushariah_voice_2012} or  authenticate the subject through behavioral characteristics, such as tactile dynamics and gait patterns\cite{collins_silhouette-based_2002,connor_biometric_2018}. Though essential, these methods are not suitable in addressing our problem due to the low-light and low-sound conditions and the subject's state of consciousness during such sleep studies.

\subsection{Radio-based Identity Verification}
Radio-based identity verification is one of among a few promising directions in addressing the aforementioned issues. It obtains unique physiological traits from radio signals reflected from the subject and does not require the subject's active involvement or ambient conditions unsuitable for the sleeping study. Several research works employ Doppler radar measurement of cardiopulmonary motion at decimeter or mmWave band for continuous user authentication \cite{ChenDopplerSignaturesRadar2008,MolchanovTargetClassificationUsing2011,RahmanNoncontactDopplerRadar2016,VanDorpFeaturebasedHumanMotion2008}. Others utilize the channel measurement protocols inherent to off-the-shelf WiFi devices to extract unique features for individual identification \cite{AbdelnasserUbiBreatheUbiquitousNoninvasive2015, LiuTrackingVitalSigns2015, ZhangWifiidHumanIdentification2016}. Recent development further incorporates advanced signal processing algorithms and machine learning techniques to improve the identification accuracy and reliability \cite{LiuContinuousUserVerificationb,IslamIdentityAuthenticationOSA2020}.

Despite many advances, two fundamental problems associated with our setting remain unsolved. First, %although the identity verification process operates on non-volitional features and require little involvement from the target users, 
the challenges to establish the connection between the radio signature and the subject's identity are largely omitted in existing work. In other words, the initial enrollment, during which the system captures the subject's physiological measurements to be compared with the traits extracted from radio signals, is contingent upon the assurance of the user's identity, which must be verified in a more reliable method. Second, the results in existing work are mostly obtained through single-subject experiments under controlled settings \cite{rahman_doppler_2018,lin_cardiac_2017,shi_contactless_2018,islam_identity_2019}. The challenges to apply radio-based approaches in complex environments subject to disruptive events and multiple targets, e.g., scenarios mostly encountered for in-home sleep arrangements, remain to be addressed.

\subsection{Co-Presence Authentication}
Another group of authentication methods applicable to test compliance tracking is co-presence verification, through which authenticator-certified devices perceive roughly the same ambient context via their on-board sensors. Context-based co-presence verification has been a long-standing challenge in security research. In \cite{ScannellProximitybasedAuthenticationMobile2009, NarayananLocationPrivacyPrivate2011, ZhengLocationBasedHandshake2017}, fluctuations in the radio signal have been used in verifying the immediate proximity between unmet/unassociated users/devices. In \cite{SchurmannSecureCommunicationBased2011, MiettinenContextBasedZeroInteractionPairing2014, HanYouFeelWhat2018, PutzAcousticIntegrityCodes2020}, mutually-observed ambient context--such as sound, luminosity, and the correlation between different sensory modalities-- have been exploited to secure the trust between legitimate parties. Since the context information are usually noisy and differ between observers, co-presence verification predominately incorporates error-tolerant algorithms to match close-to but not identical data. Common techniques include distance-bounding protocols \cite{SingeleeLocationVerificationUsing2005}, fuzzy extractor \cite{NarayananLocationPrivacyPrivate2011, ZhengLocationBasedHandshake2017}, and commitment schemes \cite{MiettinenContextBasedZeroInteractionPairing2014}, and machine learning classifiers \cite{WuLearningDevicePairing2018}. 

There exist two antithetical issues regarding context-based co-presence verification, however. On one hand, momentary snapshots of the ambient context contain little entropy to be robust against forgery or brute-force attacks. In our case, the intrinsic entropy of a person's short-term breathing pattern can be as low as 3 bits (based on our empirical analysis),  which is significantly lower than the entropy level required for security credentials. On the other hand, long-term observations of the ambient context may increase the randomness of the shared experience, but require strict data synchronization and processing techniques to extract usable fingerprints that serve as proof of sustained co-presence among devices.

==> src/sections/sienna_conf.tex <==
% \begin{figure*}[t]
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth]{figures/ChestbandDoctor.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth]{figures/OnBed.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth]{figures/InBed.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth]{figures/OutofRange.png}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.19\textwidth}
% \includegraphics[width=\textwidth]{figures/Verification.png}
% \end{subfigure}
% \caption{Left to right: (a) Doctor places chestband on patient \& pairs with app; (b) At home: the modality switch \& key evolution made possible by shared observation of patient from two sentinels; (c) mmWave radar handles compliance tracking \& data collection of patient; (d) App alerts user if they are nearing the range limit of the mmWave radar; (e) Doctor verifies compliance tracking \& checks data for any abnormalities.}
% \label{fig:mascot overview}
% \end{figure*}

% \begin{figure*}[t]
% \hspace{\fill}
% \begin{subfigure}[t]{0.28\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/doppler_radar_v1.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.28\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/system_overview.eps}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.28\textwidth}
% \includegraphics[width=\textwidth,height=\textwidth]{figures/feature_extraction_fuzzy_extractor.png}
% \end{subfigure}
% \hspace{\fill}
% \end{figure*}

\begin{figure*}[t]
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/clinic_visit.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/pairing.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/mod_change.eps}
\end{subfigure}
\hspace{\fill}
\begin{subfigure}[t]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/verification.eps}
\end{subfigure}
\caption{Left to right: (a) In hospital: a medical technician places a respiratory belt on a user and pairs it with the user's phone; (b) At home: a user pairs the PRMS with the user's phone; (c) User switches to PRMS for OSA screening; (d) Doctor verifies OSA data for any abnormalities.}
\label{fig:sienna overview}
\end{figure*}

We present SIENNA: in\textbf{SI}der r\textbf{E}sista\textbf{N}t co\textbf{N}text-based p\textbf{A}iring. SIENNA leverages the user's respiratory patterns observed by both the respiratory belt and the PRMS. To defense against an insider attack, SIENNA employs a combination of fuzzy matching and friendly jamming to prevent a non-compliant user from obtaining the pairing key using the same context.

\subsection{Overview}
The pairing procedure of SIENNA is shown in Fig. \ref{fig:sienna overview}. It begins when the user visits a doctor to obtain the test authorization. During the visit, the doctor attaches a respiratory belt to the patient, and pairs it to the user's mobile device OSA app (Fig. \ref{fig:sienna overview}a). Once arriving home, the user lies in bed and the PRMS automatically pairs with the mobile device based on the respiration pattern observed by both the PRMS and the respiratory belt (Fig. \ref{fig:sienna overview}b). Once the pairing completes, both links from the PRMS and respiratory belt to the mobile device are secure. The user can freely choose either the respiratory belt or PRMS for OSA screening, and the selected modality communicates encrypted OSA data to the mobile device (Fig. \ref{fig:sienna overview}c). Once testing is completed, the user revisits the doctor and uploads the OSA screening from the mobile device. The doctor runs a compliance check and examines whether there were any significant gaps or inconsistencies with the OSA data. Based on the compliance check report, the doctor decides whether to accept or reject the OSA screening (Fig. \ref{fig:sienna overview}d).

\subsection{Insider Resistant Device Pairing}
\label{section:key evolution}
The core of SIENNA is a context-based secure key establishment (Fig. \ref{fig:key evolution_diag}), which allows two devices, $a$ and $b$, to securely exchange and update a symmetric key in the presence of a nearby eavesdropper by utilizing the context (user's breathing patterns) observed by both devices at the moment of exchange. In the OSA scenario above, $a$ represents the mobile device connected to a respiratory belt, $b$ represents the PRMS.

\begin{figure}[h]
\centering
\includegraphics[width=0.65\linewidth]{figures/protocol.eps}
\caption{Pairing protocol for two devices observing similar data to establish a symmetric key in the presence of an adversary.}
\label{fig:key evolution_diag}
\vspace{-10pt}
\end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.75\linewidth]{figures/Quantization-of-Signal.png}
% \caption{Encoding of a breathing pattern signal \& generation of a key using level-crossing quantization.}
% \label{fig:level-crossing quantization}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.75\linewidth]{figures/Protocol.jpg}
% \caption{Key evolution protocol for two devices that share the same observed data to establish a symmetric key in the presence of an adversary.}
% \label{fig:key evolution}
% \end{figure}

Traditional context-based key establishment protocols are not secure when eavesdroppers are nearby to observe the context. Many of such protocols assume that the adversary cannot be near paring devices over extended periods of time \cite{MiettinenContextBasedZeroInteractionPairing2014}. SIENNA addresses this shortcoming through a cross-layer design that employs two security primitives: fuzzy commitment \cite{JuelsFuzzyCommitmentScheme1999} and and dialog-codes-based friendly jamming \cite{AroraDialogCodesSecure2009,GollakotaPhysicalLayerWireless2011, MelcherIJamChannelRandomization2020}. The former is a cryptographic scheme that allows secure commit and de-commit of a secrete similar-but-not-identical open value. The latter is a friendly jamming scheme at the receiver by jamming the transmitted signal to flip specific bits in the message. Together, this ensures that an eavesdropper with the right context will not be able to recover the key exchanged between the pairing devices.

First we define the fuzzy commitment scheme \cite{JuelsFuzzyCommitmentScheme1999}. Let $\sigma$ be a secret value. A fuzzy commitment transforms a secret value $\sigma$ into a commitment $\{\chi, \mathcal{H}(\sigma)\}$ using an opening feature, $\phi$, and a hash function, $\mathcal{H}(\cdot)$:
\[
\{\chi, \mathcal{H}(\sigma)\} = \textsc{Commit}(\sigma, \phi),
\]
such that $\chi$ appears random and devoid of any information about $\sigma$. And all open features $\hat{\phi}$ reveals $\sigma$ via 
\[
\sigma=\textsc{Open}(\chi,\hat{\phi}),
\]
if and only if the Hamming distance $\textsc{Ham}(\phi, \hat{\phi}) \leq \tau$, where $\tau$ is a parameter denoting the maximum allowable Hamming distance between $\hat{\phi}$ and $\phi$ to reveal $\sigma$. 

To initiate the key establishment protocol, $a$ broadcasts a message, $\{ \mathcal{H}(k), t_{\text{str}}, t_{\text{end}} \}$, where $k$ denotes the key of the previous iteration. $t_{\text{str}}$ and $t_{\text{end}}$ denotes the starting and ending timestamps of $a$ and $b$'s captures of the respiratory patterns. During the first round,  $\mathcal{H}(k)$ is replaced with a public parameter known to all parties.

From respiratory patterns $r_{a}(t_{\text{str}}, t_{\text{end}})$ and $r_{b}(t_{\text{str}}, t_{\text{end}})$ captured within the specified time interval, the two devices extract breathing fingerprints $f_{a} = \textsc{Ext} \left( r_{a}(t_{\text{str}}, t_{\text{end}}) \right)$ and $f_{b} = \textsc{Ext} \left( r_{b}(t_{\text{str}}, t_{\text{end}}) \right)$, via a fingerprint extraction function $\textsc{Ext} (\cdot): \{1,0\}^{*} \mapsto \{1,0\}^{M*2^K}$ (detailed in Sec. \ref{section:respiration fingerprinting}). In case $a$, e.g., PRMS, observes a breathing mixture of multiple subjects, the mixture is first separated into the breathing patterns of individual subjects (detailed in Sec. \ref{section:breathing separation}), which are processed by $\textsc{Ext} (\cdot)$ to create multiple fingerprints, one for each subject.

Once the breathing fingerprints are generated, $a$ randomly selects a key salt, $ s \in \{1,0\}^{N*2^K}$, and transforms it into a commitment $\{c \in \{1,0\}^{M*2^K}, \mathcal{H}(s)\}$ using the breathing fingerprint, $f_{a}$. Specifically, $a$ encodes $s$ via the Reed-Solomon (RS) encoding function
\[
l = \textsc{RS}(2^K, M, N, s) \in \mathbb{F}^M_{2^K}
\]
and compute:
\[
c = l \ominus f_{a},
\]
with $\ominus$ denoting exclusive OR (XOR).

Henceforth, $a$ and $b$ exchange $c$ through dialog codes to defend against insider attack. First, $a$ converts the commitment,
\[
\{c, \mathcal{H}(s)\},
\]
into OFDM symbols, duplicates each symbol back-to-back,
\[
\textsc{DupSym}\left(\{c, \mathcal{H}(s)\}\right),
\]
and broadcasts all the symbols. In parallel to $a$'s broadcast, $b$ randomly jams either the original symbol or its repetition \cite{GollakotaPhysicalLayerWireless2011,AroraDialogCodesSecure2009}, 
\[
\textsc{PhyJam}\left(\|\textsc{DupSym}\left(\{c, \mathcal{H}(s)\}\right)\|\right),
\]
To jam a symbol, $b$ transmits a signal that is drawn randomly from a zero-mean Gaussian distribution whose variance is the same as the OFDM signal with the same modulation. Since $b$ knows which symbols are jammed, it stitches the unjammed symbols together to create a clean version of the OFDM transmission and decodes the signal to obtain the clear message.

Upon receiving $\{c, \mathcal{H}(s)\}$, $b$ computes 
\[
\hat{l} = f_{b} \ominus c
\]
and decommits the salt by decoding $\hat{l}$ using the Reed-Solomon (RS) decoding function: 
\[
\hat{s} = \overline{RS}(2^K, M, N, \hat{l}).
\]
Due to the error correction capability of Reed–Solomon codes, $s$ equals to $ \hat{s}$ if and only if $l$ and $\hat{l}$ differ in less than $2^{K-1}(M-N)$ bits. Since $l = f_{a} \ominus d$ and $\hat{l} = f_{b} \ominus d$, it is equivalent in saying that $f_{a}$ and $f_{b}$ must differ in less than $T$ bits for $b$ to retrieve $s$.

To confirm whether the retrieval were successful, $b$ computes $\mathcal{H}(\hat{s})$ and compares it with $\mathcal{H}(s)$. Depending on whether they were equal, an $\textsc{ACK}$ or a $\textsc{NAK}$ message is transmitted from $b$ to $a$, with the former initiating the final step of the key establishment protocol and the latter initiating the reattempts.

To conclude the key establishment, both $a$ and $b$ applies a key derivation function 
\[
k' = \textsc{KDF}(k, s),
\]
to obtain the new key.

\subsection{Breathing Separation with JADE-ICA}
\label{section:breathing separation}
Home environments are noisy and unpredictable, with the possibility of irrelevant individuals in close vicinity from the user. To retrieve the correct context in an environment with potentially multiple subjects, SIENNA augments the PRMS modality with a breathing separation module, which reconstructs the breathing signals of multiple co-located individuals to select the correct target. 
%The wireless (mmWave radar) modality in our compliance tracking system is particularly susceptible to such complications, as the RF reflections off the bodies would superimpose over the wireless medium and interfere at the receiver.
% Several works have been proposed to correctly separate and isolate the patient's respiratory signature from the combined signal mixture, all of which fall into the problem domain of blind source separation (BSS) \cite{yue_extracting_2018,petrochilos_blind_2007,cardoso_blind_1998,de_lathauwer_independent_1996,rutledge_independent_2013}. 
The goal of the separation module is to reconstruct a set of source signals from a set of mixtures, without knowing the properties of the sources and the mixing proportion. 
%A common example of such BSS is the cocktail party problem where multiple people's voice signal is mixed into the speaker and need to be separated \cite{yue_extracting_2018,petrochilos_blind_2007,cardoso_blind_1998}. 
Since respiration signals are non-Gaussian and independent from individuals, whilst mixed linearly at the PRMS receiver, one can recover the source signals using independent component analysis (ICA) \cite{yue_extracting_2018}, which is formulated as the following: assume $N$ independent time varying sources $ s_i(t),\ i=1 \ldots N$, and $M$ different observations
$ x_i(t),\ i=1 \ldots M$. For $T$ time units $(t=1 \ldots T)$, we can define the source signal as a $N \times\ T$ matrix,
\[
\mathbf{S}_{N \times T} = \begin{bmatrix} 
    s_{11} & s_{12} & \dots \\
    \vdots & \ddots & \\
    s_{N_1} &        & s_{N_T} 
    \end{bmatrix},
\]
and the observed mixtures as a $M \times\ T$ matrix,
\[
\mathbf{X}_{M \times T} = \begin{bmatrix} 
    x_{11} & x_{12} & \dots \\
    \vdots & \ddots & \\
    x_{M_1} &        & x_{M_T}
    \end{bmatrix}.
\]
The mixtures are produced as the product of the source and a mixing matrix $\mathbf{W}_{M \times N}$, e.g.,
\[
    \mathbf{X}_{M \times T} = \mathbf{W}_{M \times N} \times \mathbf{S}_{N \times T}.
\]
The goal of ICA is to recover $\mathbf{S}_{N \times T}$ and $\mathbf{W}_{M \times N}$ given only $\mathbf{X}_{M \times T}$, assuming
the $s_i(t),\ i=1 \ldots N$ are independent and non-Gaussian. We employ the joint approximate diagonalization of eignematrices (JADE) algorithm \cite{de_lathauwer_independent_1996} to perform ICA, with the details omitted to conserve space\footnoteref{tech_report}. 

% The JADE algorithm extracts independent non-Gaussian sources $\mathbf{S}_{N \times T}$, e.g., the breathing pattern of individual targets, from signal mixtures with Gaussian noise $\mathbf{X}_{M \times T}$, e.g., the breathing mixture received by the radar sentinel, by constructing a fourth-order cumulants array from $\mathbf{X}_{M \times T}$. Specifically, assuming $T > M,N$, the algorithm first applies PCA to whiten $\mathbf{X}_{M \times T}$, resulting
% \[
% \mathbf{P}^{\text{tr}}_{T \times K} = \mathbf{B}_{K \times M} \times \mathbf{X}_{M \times T},
% \]
% with a whitening matrix $\mathbf{B}_{K \times M}$.
% %has $N$ rows with $N$ being the number of singular values of $\mathbf{X}_{M \times T}$, and $M$ the columns of whitened matrix $\mathbf{P}_{T \times N}$ are orthogonal with equal variance. 
% After the whitening, the columns of whitened matrix $\mathbf{P}_{T \times K}$ are orthogonal with equal variance. Any rotation of $\mathbf{P}_{T \times K}$ will not change the independence between it column vectors. The algorithm then tries to find a rotation matrix $\mathbf{V}_{N \times N}$ to maximize the independence between the row vectors of the rotated $\mathbf{P}_{T \times K}$, which is achieved when the fourth-order cross-cumulants between the row vectors are zero and their auto-cumulants maximal. Once $\mathbf{V}_{N \times N}$ has been identified, the demixing matrix can be computed as 
% \[
%     \mathbf{W}^{+}_{N \times M} = \mathbf{V}_{N \times N} \times \mathbf{B}_{N \times M},
% \]
% and the source matrix as
% \[
%     \mathbf{S}_{N \times T} = \mathbf{W}^{+}_{N \times M} \times \mathbf{X}_{M \times T},
% \]
% More detailed information on JADE and cumulant tensor array can be found at \cite{rutledge_independent_2013} and the Matlab code on the website \cite{CardosoBlindSeparationReal}.
%  {\ \ \ \ \ \ \ a}_{M\times T}=\ \left[\begin{matrix}a_{11}&\cdots&a_{1M}\\\vdots&\ddots&\vdots\\a_{M1}&\cdots&a_{MT}\\\end{matrix}\right]
 
%  The observations are written as \(M\times\ T\) matrix. 
 
%  {\ \ \ \ \ \ \  s}_{N\times T}=\ \left[\begin{matrix}s_{11}&\cdots&s_{1N}\\\vdots&\ddots&\vdots\\s_{N1}&\cdots&s_{NT}\\\end{matrix}\right]
 
%  Basically, the observation is produced by combining source signal \(a_{M\times T}\) via mixing matrix \(W_{N\times M}\), such that we can write  \( s_{N\times T}=W_{N\times M}\times\ a_{M\times T}\). The goal of ICA is to recover pure source signal from their independence properties by extracting demixing matrix which is represented as \(W_{N\times M}^{-1}\): \(a_{M\times T}=W_{N\times M}^{-1}\times\ s_{N\times T}\). In literature, there are different ICA algorithms, among them fast ICA, Infomax and joint approximate diagonalization of eignematrices (JADE) is most popular \cite{de_lathauwer_independent_1996}. JADE is fourth order statistics kurtosis based ICA method \cite{cardoso_blind_1998,de_lathauwer_independent_1996,rutledge_independent_2013}. The main advantages of this technique is that it is matrix diagonalization based approach whereas other algorithm depends on optimization procedure and hence variable results might occur \cite{cardoso_blind_1998,de_lathauwer_independent_1996,rutledge_independent_2013}. In our previous reported results we tested the efficacy of JADE algorithm for separating respiratory signatures from combined mixture of signals \cite{islam_separation_2018,islam_multiple_2019}. 

\subsection{Fingerprinting with Level-Crossing Quantization}
\label{section:respiration fingerprinting}

% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.23\textwidth}
% \includegraphics[width=\textwidth]{figures/Protocol.jpg}
% \end{subfigure}
% \hspace{\fill}
% \begin{subfigure}[t]{0.23\textwidth}
% \includegraphics[width=\textwidth]{figures/Quantization-of-Signal.png}
% \end{subfigure}
% \caption{(a) Key evolution protocol for two devices that share the same observed data to establish a symmetric key in the presence of an adversary; (b) Encoding of a breathing pattern signal \& generation of a key using level-crossing quantization.}
% \label{fig:sienna}
% \end{figure}

Once the devices obtain breathing patterns of individual targets, they apply $\textsc{Ext} (\cdot)$ to extract the binary breathing fingerprints. The binary strings must meet two criteria for the two to agree on the patient's identity and evolve the shared security key: (1) they should look sufficiently similar in Hamming space if they represent the breathing process of the same person, and (2) they should preserve the uniqueness of the breathing dynamic that distinguishes among individuals.

To achieve these objectives, $\textsc{Ext} (\cdot)$ applies level-crossing quantization to sample the continuous breathing patterns with two predefined thresholds. Let $q_{+}$, $q_{-}$ be the thresholds values such that $q_{+} > q_{-}$, we define a quantizer $\textsc{Qtz} (\cdot)$:
\begin{equation*}
  \setlength{\arraycolsep}{0pt}
    \textsc{Qtz} (x) = \left\{ \begin{array}{ l l }
    10 &\;\;\;\;\text{if}\; x \geq q_{+} \\
    01 &\;\;\;\;\text{if}\; x \leq q_{-} \\
    00 &\;\;\;\;\text{if}\; q_{-} < x < q_{+}
  \end{array} \right.
\end{equation*}
Let $T$ be the time interval between adjacent sampling instants. The binary sequence obtained by $\textsc{Ext} (\cdot)$ is
\begin{multline*}
f = \textsc{Ext} \left(r(t_{\text{str}}, t_{\text{end}})\right) = [\textsc{Qtz} \left( r(t_{\text{str}}) \right),...,\\
    \;\;\;\;\;\;\;\textsc{Qtz} \left(r(t_{\text{str}} + \lfloor\frac{t_{\text{end}} - t_{\text{str}}}{T}\rfloor T \right)],
\end{multline*}
which can be compared in Hamming space.
% If the binary sequence is longer than the length of the commitment,  $\|\lambda\|$, we pad and divide it into multiple subsequences, $f = [ f_1, f_2,...,f_n]$ to commit
% \begin{equation}
% c = f_1 \ominus f_2 \ominus ... \ominus f_n \ominus l,
% \end{equation}
% and decommit
% \begin{equation}
% \hat{l} = \hat{f}_1 \ominus \hat{f}_2 \ominus ... \ominus \hat{f}_n \ominus c,
% \end{equation}
% The level-crossing quantization described above is an event-based sampling procedure as the crossing events are encoded as changes in the binary patterns. When the signal remains above/below the levels, it produces fixed patterns, which can be exploited to further compress the binary before transmission\footnote{Techniques to produce a compressed the binary string that are satisfiable to the two criteria is beyond the scope of this article and will be investigated in the future.}. 


However, the result of a single level-crossing quantization loses details in the original breath pattern and fails the second objective. To address this issue, we apply multiple passes of level-crossing binary quatizations, each at a distinct pair of levels, $q_{i+}$, $q_{i-}$. Intuitively, it is equivalent to create a pair-wise linear approximation of the original breathing pattern, with quantization error equal to the level density.

If the binary fingerprints after the multi-level quantization is longer than $\|l\|$, we pad and divide it into multiple subsequences, $f = [ f_1, f_2,...,f_n]$ to commit
\[
c = f_1 \ominus f_2 \ominus ... \ominus f_n \ominus l,
\]
and decommit
\[
l = f_1 \ominus f_2 \ominus ... \ominus f_n \ominus c.
\]

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.65\linewidth]{figures/Quantization-of-Signal.png}
% \caption{Encoding of a breathing pattern signal \& generation of a key using level-crossing quantization.}
% \label{fig:quantization}
% \end{figure}
%Since the human breathing signal is bandlimited, we can eliminate alias in the approximation by setting the sampling frequency to above the Nyquist rate.

% \subsection{The MASCOT Scheme}
% The detailed design of MOTIVE is shown in Figure XXX. Once being recommended to undergo the OSA screening, the patient first visits his/her doctor to obtain the test authorization. During the visit, his/her doctor attaches the chest band sensor to the patient and input a signature key to the storage module onboard the sensor. The sensor continuously record the patient's respiratory patterns from the moment it is attached. Any attempts to remove the sensor nullifies the test. For each record, the sensor labels it with a timestamp and store it in the tamper-proof storage module. The OSA screening system broadcasts a \texttt{READY} message, and waits for the signals from the sensor.

% Upon receiving the \texttt{READY} message, the chest band sensor alerts the patient the possibility of modality switch. If the patient wishes to switch the mode, the sensor generates a random session key. It encapsulates the session key and the signature key in a fuzzy extractor built from the patient's most recent respiratory patterns and broadcasts the encapsulation. Upon receiving the message, the OSA screening system attempts to reconstruct both keys with the respiratory patterns collected by the mmWave radar. If there were multiple persons in the room, the OSA screening system tries individual signal traces to find the one that matches the fuzzy extractor. If the key establishments were successful, the OSA screening system acknowledges the transition by replying an \texttt{ACK} message encrypted via the session key. Once the message is decrypted and verified, the chest band sensor transfers its data records securely using the session key and notify the patient of the modality change. The patient may take off the chest band sensor. The OSA screening system signs the data records transferred from the sensor and continue on the recording and signing tasks.

% If the patient is about to move out-of-view from the radar and the radar signals degrade, the OSA screening system notifies the patient to reattach the chest band sensor. Once attached, the chest band sensor reactivates and broadcasts a \texttt{READY} message, and waits for the signal from the by OSA screening system. Upon receiving the \texttt{READY} message, the OSA screening system generates a random session key, encapsulates it in a fuzzy extractor, and initiates the key agreement protocol with the chest band sensor. If the sensor were able to extract and verify the session key, the sensor acknowledges the OSA screening system by replying to an \texttt{ACK} message encrypted by the session key and resume the recording, with the OSA screening system entering the idle mode. The chest band sensor needs to remain attached until the next modality switch. Any attempts to remove the sensor during that period also nullifies the test.

% Modality switching can occur multiple times throughout the test. Once the test completes, the patient's doctor collects the respiratory pattern records from the OSA screening system and run an automatic validity check to examine whether there were significant gaps or inconsistencies between the data entries. Based on the report of the validity check, the doctor decides whether to accept or reject the sleep test.

% arythom it works  methods for 
% Basically, by measuring the phase shift of the reflected radar signal induced by tiny movement of the chest surface due to cardio-respiratory activity breathing rate and heart rate can be extracted remotely \cite{droitcour_microwave_2001,lin_microwave_1992,chen_x-band_1986,lin_noninvasive_1975,greneker_radar_1997,droitcour_non-contact_2009,singh_data-based_2013}. Compared with other proposed conventional biomedical radars based identity authentication system that can only authenticate single subject \cite{lin_cardiac_2017,rahman_doppler_2018,shi_contactless_2018,islam_identity_2019}, the main novelty of the proposed technique is to isolate respiratory pattern from combined mixture by having concurrent measurement of two subjects with the field of view of radar using ICA-JADE algorithm. In our proposed authentication system, if there is multiple subject present in front of the radar then radar gets combined mixture so we integrated ICA-JADE algorithm to isolate independent respiratory signature from combined mixture \cite{islam_separation_2018}. After separating independent respiratory signatures, we extracted respiratory breathing related dynamic features (breathing rate, peak distribution, breathing energy,spectral entropy, inhale area and exhale area). We also integrated machine learning classifiers with the hyper-feature set and combined Fuzzy Extractor with linear coding to transform the hyper-feature sets into strong biometric keys. 

% A typical Doppler radar transceiver transmits electromagnetic signal and demodulates the signal reflected back from human. According to Doppler theory, the phase of the reflected signal is directly proportional to the tiny movement of the chest surface due to cardio-respiratory activity \cite{lin_noninvasive_1975,lin_noninvasive_1975}. A typical direct conversion CW quadrature channel radar evaluates into the following baseband equations \cite{droitcour_microwave_2001,singh_data-based_2013}: 

%  Where, two above equations represent in-phase and quadrature-phase of the demodulated signal. Here, x(t) is the chest displacement, \(\lambda\) is the wavelength,\(A_{BI}\), \(A_{BQ}\) is the amplitude and \(∆\phi(t)\) is the phase noise of the oscillator. Before demodulating the signal, we used to correct channel imbalance of I/Q signal \cite{singh_data-based_2013}. Then we plot the corrected baseband signal \(B_{Ic}(t)\) and \(B_{Qc}(t)\) against each other on complex plane which is I/Q plot \cite{singh_data-based_2013}. A center estimation algorithm is employed to find radius of arc and center of the arc origin \cite{singh_data-based_2013}. Two different type of demodulation technique is generally employed for extracting phase information of the signal \cite{droitcour_microwave_2001}. One is linear demodulation and another one is arc-tangent demodulation \cite{singh_data-based_2013}. After utilizing demodulation technique, we can extract chest wall displacement information which is represented below in equation \cite{droitcour_microwave_2001}. 

% {\ \ \ \ \ \ \ \ \ \ \ \ \theta}\left(t\right)=\frac{4\pi x\left(t\right)}{\lambda}

% Where, \(\theta(t)\) represents the angle formed by the arc in IQ plane. The tiny chest displacement is directly proportional to the phase change of the reflected signal \cite{singh_data-based_2013}. 
